An agent design with goal reaching guarantees for enhancement of learning

Reinforcement learning is commonly concerned with problems of maximizing accumulated rewards in Markov decision processes. Oftentimes, a certain goal state or a subset of the state space attain maximal reward. In such a case, the environment may be considered solved when the goal is reached. Whereas numerous techniques, learning or non-learning based, exist for solving environments, doing so optimally is the biggest challenge. Say, one may choose a reward rate which penalizes the action effort. Reinforcement learning is currently among the most actively developed frameworks for solving environments optimally by virtue of maximizing accumulated reward, in other words, returns. Yet, tuning agents is a notoriously hard task as reported in a series of works. Our aim here is to help the agent learn a near-optimal policy efficiently while ensuring a goal reaching property of some basis policy that merely solves the environment. We suggest an algorithm, which is fairly flexible, and can be used to augment practically any agent as long as it comprises of a critic. A formal proof of a goal reaching property is provided. Comparative experiments on several problems under popular baseline agents provided an empirical evidence that the learning can indeed be boosted while ensuring goal reaching property.

==> input/abstract.tex <==
Reinforcement learning is commonly concerned with problems of maximizing accumulated rewards in Markov decision processes.
Oftentimes, a certain goal state or a subset of the state space attain maximal reward.
In such a case, the environment may be considered solved when the goal is reached.
Whereas numerous techniques, learning or non-learning based, exist for solving environments, doing so optimally is the biggest challenge.
Say, one may choose a reward rate which penalizes the action effort.
Reinforcement learning is currently among the most actively developed frameworks for solving environments optimally by virtue of maximizing accumulated reward, in other words, returns.
Yet, tuning agents is a notoriously hard task as reported in a series of works.
Our aim here is to help the agent learn a near-optimal policy efficiently while ensuring a goal reaching property of some basis policy that merely solves the environment.
We suggest an algorithm, which is fairly flexible, and can be used to augment practically any agent as long as it comprises of a critic.
A formal proof of a goal reaching property is provided.
Simulation experiments on six problems under five agents, including the benchmarked one, provided an empirical evidence that the learning can indeed be boosted while ensuring goal reaching property.

==> input/approach.tex <==
Recall the problem setup of \Cref{sec_problem}.
Let, for the sake of motivation, the reward function to be negative-definite \ie $\robj(0,0)=0, \robj<0$ otherwise.
In general, it holds, by the virtue of the Hamilton-Jacobi-Bellman (HJB) equation, that $\forall t \ge 0 \spc \Value^*_{t+1} - \Value^*_t = -\robj^*_t$, where the optimal value satisfies $\Value^*_t := \E[\Action_t \sim \policy^*(\bullet \mid \state_t), \State_{t+1} \sim \transit( \bullet \mid \state_t, \Action_t ) ]{\robj(\state_t, \Action_t) + \Value^{\policy^*} \left( \State_{t+1} \right)}$, and $\robj^*_t := \E[\Action_t \sim \policy^*]{\robj(\state_t, \Action_t)}$.
Here, it was assumed that the problem was undiscounted \ie $\gamma = 1$ for motivational purposes.
Essentially, the HJB dictates that any specified goal $\G \supset 0$ is reached, generally in a probabilistic sense, by the agent following the optimal policy because (1) $\Value^*$ is finite for any initial state, (2) $\Value^*_t$ is strictly increasing due to $r$ being negative-definite.
If a model \ie a critic, is employed \eg a $w$-weighted deep neural network $\hat \Value^w(\state)$, then due to imperfections of learning, the goal reaching property may be lost, yet it is desired.
It is tempting to ask on retaining the said property.
Unfortunately, no such guarantee can be given under learned critic and policy models in practice.
The hypothesis of this work is that if the agent is supported by a policy $\policy_0 \in \policies_0$ (see \Cref{sec_problem}), such a guarantee can be provided which in turns improves the learning.
As discussed in \Cref{sec_problem}, just finding a policy $\policy_0 \in \policies_0$ is not a difficult task which can be accomplished by various techniques \cite{Johnson2005PIDcontrol,Perruquetti2002SlidingModeCo,vaidyanathan2017applications,Zhu2006Flatnessbased,Berger2021Funnelcontrol}.
The challenge is to find the optimal policy $\policy^*$, which is the aim of the agent.
The idea here is to build on top of a nominal agent, which could in turn be based on any reinforcement learning algorithm with a critic, and to prioritize those critic updates which exhibit the property of the kind $\hat \Value^w(\state_{t+1}) - \hat \Value^{w^\dagger}(\state_t^\dagger) > 0$, where the weight tensor $w^\dagger, \state_t^\dagger$ are yet to be determined.
Namely, the critic update is done so as to try to satisfy the said property.
Should this be the case, the optimized weights are assigned to $w^\dagger$ and the current state is assigned to $\state_t^\dagger$.
Subsequently, the action generated by the actor's policy $\policy$ is applied to the environment.
If the critic update did not satisfy the condition $\hat \Value^w(\state_{t+1}) - \hat \Value^{w^\dagger}(\state_t^\dagger) > 0$, then the action generated by $\policy_0$ is applied.
Notice that even if there are to policies $\policy_0, \policy'_0$ with a goal reaching property \ie $\policy_0, \policy'_0 \in \policies_0$, it is not the case that an arbitrary switching between $\policy_0$ and $\policy'_0$ has the goal reaching property.
Hence, combining policies is generally not trivial.
We overcome this difficulty in the herein presented approach by ``freezing'' the critic $\hat \Value^{w^\dagger}$ if it failed to satisfy $\hat \Value^w(\state_{t+1}) - \hat \Value^{w^\dagger}(\state_t) > 0$.
In \Cref{sub_contrib}, we stated that such an approach was not to be necessarily seen as a direct alternative to the existing baselines.
This is because, as long as the agent comprises of a critic part, the current approach puts no restrictions on the choice of the actor and critic loss functions $\loss_\act$ and $\loss_\crit$, respectively; optimization routines; schedules to update (online or episodic Monte-Carlo); models; replay buffer accumulation and sampling algorithms etc.
Now, besides $\hat \Value^w(\state_{t+1}) - \hat \Value^{w^\dagger}(\state_t) > 0$, the critic should also satisfy the property $- \hat \kappa_\up (\nrm{\state_t}) \le \hat \Value^{w}(\state_t) \le - \hat \kappa_\low(\nrm{\state_t})$, where $\hat \kappa_\up, \hat \kappa_\low: \R_{\ge0} \ra \R_{\ge0}$ are two functions which are zero at zero, monotonically increasing and tending to infinity.
Their choice is fairly loose \eg
\begin{equation}
	\label{eqn_calf_quadkapps}
	\hat \kappa_\low(x) = C_\low x^{2}, \ \hat \kappa_\up(x) = C_\up x^{2}, \spc 0 < C_\low < C_\up \text{ arbitrary},
\end{equation}
is acceptable.
One may \eg square the output of the critic network and add a small regularization while putting any a priori fixed lower and upper bound on the weights \ie the weights lie in some compact $\W$.
The reason is that we do not want the critic to be arbitrarily negative large and, respectively, small for non-zero states (equivalently, states outside $\G$).
Finally, the condition $\hat \Value^w(\state_{t+1}) - \hat \Value^{w^\dagger}(\state_t^\dagger) > 0$ should be cast into a non-strict one with any $\bar \nu > 0$ in place of the zero.
In \Cref{alg_calfstate}, we present a fairly generic, online form of the suggested approach.

\begin{algorithm}
	\begin{algorithmic}[1]
		\STATE {\bfseries Setup:} MDP, nominal agent details \eg networks, actor loss function $\loss_\act$, critic loss function $\loss_\crit$, and ${\bar \nu} > 0, \hat \kappa_\low, \hat \kappa_\up, \policy_0 \in \policies_0$
		\STATE \textbf{Initialize}: $\state_0, w_0 \in \W$
		\STATE $w^\dagger \gets w_{0}, \state^\dagger \gets \state_0$ 
		\FOR {$t := 1, \dots \infty$}
			\STATE Take action sampled from $\policy_{t-1}(\bullet \mid \state_{t-1})$, get state $\state_t$
			\STATE Try critic update \alglinelabel{algline_calfcrit}
			\[
				\begin{array}{lrl}
					w^* \gets & \argmin \limits_{w \in \mathbb W} & \loss_\crit(w) \\
					          & \sut                              & \hat \Value^w(\state_t) - \hat \Value^{w^\dagger}(\state^\dagger) \ge \bar \nu \\
					          &                                   & -\hat \kappa_\up(\nrm{\state_t}) \le \hat \Value^{w}(\state_t) \le -\hat \kappa_\low(\nrm{\state_t})
				\end{array}
			\]
			\IF{ solution $w^*$ found}	\alglinelabel{algline_calfcheck}
				\STATE $\state^\dagger \gets \state_t, w^\dagger \gets w^*$
				\STATE	Update policy: \alglinelabel{algline_calfact}
				\[
					\policy_{t}(\bullet \mid \state_{t}) \la \argmin\limits_{\policy \in \policies} \loss_\act(\policy)
				\]		
				If desired, $\policy_{t}$ may be taken to produce a random action with probability $\eps>0$		 
				\ELSE
				\STATE $\policy_{t}(\bullet \mid \state_{t}) \gets \policy_0(\bullet \mid \state_t)$	
			\ENDIF	
		\ENDFOR
	\end{algorithmic}
	\caption{Suggested goal reaching agent (state-valued critic).}
	\label{alg_calfstate}
\end{algorithm}

%Let $\G$ be a compact neighborhood of the origin.
The main goal reaching result related to \Cref{alg_calfstate} is formulated in \Cref{thm_calfstabmean}.

\begin{thm}
	\label{thm_calfstabmean}
	Consider the problem \eqref{eqn_value} under the MDP \eqref{eqn_mdp}.
	Let $\policy_{0} \in \policies_0$ have the goal reaching property for $\G \subset \states$ \ie
	\begin{equation}
		\label{eqn_stabilization_inthm}
%		\policy_0 \in \policies_0 \implies
		\begin{aligned}
			& \lim\limits_{t \ra \infty}\E[\policy_0]{\goaldist(\State_t)} = 0, \\
			& \forall \eps>0 \spc \exists \delta \ge 0 \spc \E{\goaldist(\State_0)} \le \delta \implies \forall t \ge 0 \spc \E[\policy_0]{\goaldist(\State_t)} \le \eps.
		\end{aligned}		
%		\lim\limits_{t \ra \infty}\E[\policy_0]{\inf\limits_{\state \in \G} \nrm{\State_t - \state} \mid \State_0 = \state_0} = 0,
	\end{equation}
	where the convergence in limit is assumed compact in $\state_0$ and $\delta$ is unbounded as a function of $\eps$.
	Let $\policy_t$ be produced by \Cref{alg_calfstate} for all $t \ge 0$.
	Then, the same goal reaching property \eqref{eqn_stabilization_inthm} is preserved under $\policy_t$.
%	Then, the goal reaching property is preserved \ie
%	\begin{equation}
%		\label{eqn_calfstabclaim}
%		\begin{aligned}
%			 \lim\limits_{t \ra \infty}\E[\policy_t]{\inf\limits_{\state \in \G} \nrm{\State_t - \state} \mid \State_0 = \state_0} = 0.
%		\end{aligned}
%	\end{equation}
\end{thm}

\begin{crl}
	\label{crl_calfstabevent}
	Let $E$ be an event that implies uniform goal reaching under $\policy_{0}$ \ie
	\begin{equation}
		\label{eqn_stabprobuniform}
  		\Action_t \sim \policy_0(\bullet \mid \state_t) \implies 
  			\begin{cases}
  				\lim\limits_{t \ra \infty}\goaldist(\State_t) = 0, \\
  				\forall \eps>0 \spc \exists \delta \ge 0 \spc \goaldist(\State_0) \le \delta \implies \forall t \ge 0 \spc \goaldist(\State_t) \le \eps,
  			\end{cases}
%  		\lim\limits_{t\rightarrow \infty}\goaldist( \State_t) = 0,
	\end{equation}
	where uniform convergence over $\omega \in E$ and $\state_{0} \in \states_0$ is implied for an arbitrary compact set $\states_0 \subset \states$, and $\delta$ is unbounded as a function of $\eps$.
	
	Then under $\policy_t$, the probability of goal reaching is no less than $\PP{E}$\ie
	\begin{equation}
				 \PP{\lim\limits_{t \ra \infty} \goaldist( \State_t) = 0 \land \forall \eps>0 \spc \exists \delta \ge 0 \spc \goaldist(\State_0) \le \delta \implies \forall t \ge 0 \spc \goaldist(\State_t) \le \eps \mid \Action_t \sim \policy_t(\bullet \mid \state_t)} \geq \PP{E}.
	\end{equation}
\end{crl}

%\begin{rem}
%The condition \eqref{eqn_stabprobuniform} can be understood practically as follows.
%
%\end{rem}

\begin{rem}
	The latter corollary implies that  \Cref{alg_calfstate} preserves the probability of goal reaching if goal reaching is not certain under $\policy_0$.
\end{rem}

The full technical details and proof of \Cref{thm_calfstabmean} are given in \autoref{sec_thms}.
Auxiliary goal reaching preservation results are also found in \autoref{sec_thms}, \Cref{lem_calfstabtract} in particular.


\begin{rem}
	\label{rem_Hoeffding}
	The policy $\policy_0$ may be either derived by techniques such as proportional-derivative-integral regulator \cite{Johnson2005PIDcontrol,Wang2020PIDcontrolsys}, sliding-mode regulator \cite{Perruquetti2002SlidingModeCo,vaidyanathan2017applications}, flatness-based regulators \cite{Zhu2006Flatnessbased}, energy-based regulators \cite{Spong1996Energybasedco}, funnel regulators \cite{Berger2021Funnelcontrol}, gain schedulers \cite{Rotondo2017Advancesgains} etc., or using environment runs over a distribution of start states $\state_0$ while employing statistical
	confidence bounds by \eg Hoeffding’s inequality in terms of the number of runs \cite{Hertneck2018Learningapprox}.
\end{rem}

\begin{rem}
	\label{rem_calfupdates}
	In \Cref{alg_calfstate}, the critic and actor updates (lines \ref{algline_calfcrit}, \ref{algline_calfact}) are fairly flexible.
	They may be varied to the user's choice without affecting the claim of \Cref{thm_calfstabmean}.
	In particular, if desired:
	\begin{enumerate}
		\item the constraints in line \ref{algline_calfcrit} may be shifted to the loss function $\loss_\crit$ as penalties;
		\item the constraints in line \ref{algline_calfcrit} may be omitted altogether and just checked in line \ref{algline_calfcheck} instead;
		\item the critic and policy updates (lines \ref{algline_calfcrit}, \ref{algline_calfact}) may be arbitrarily event triggered.
		In the given listing, the updates are done at every step $t$, but the they may also be triggered upon episode ends (cf. Monte-Carlo updates).
	\end{enumerate}
\end{rem}

\begin{rem}
	\label{rem_calfnogoal}
	Notice no direct specification of the goal $\G$ is required in \Cref{alg_calfstate}. 
\end{rem}

\begin{rem}
	\label{rem_calfstabclaim}
	The claim of \Cref{thm_calfstabmean} can be rephrased in the following way: $\state_t$ will eventually get arbitrarily close to $\G$ in mean and stay there permanently.
	In simpler terms \autoref{thm_calfstabmean} states that \Cref{alg_calfstate} computes a policy that is guaranteed reach the goal in a suitable statistical sense.
	This result is valuable, because it indicates that even a poorly trained reinforcement learning agent will still reach the goal with guarantee in all learning episodes.
	The hypothesis, which was supported by the experiments of this work, is that such a guarantee helps boost learning.
\end{rem}

\begin{rem}
	\label{rem_policymodel}
	In practice, the policy will usually be represented as some $\theta$-weighted model \eg softmax or Gaussian, in which case the policy update would actually mean the weight $\theta_t$ update.
	In case of a Markov policy, one directly updates the action $\action_t$.
\end{rem}

==> input/bgproblem.tex <==
Consider the following Markov decision process (MDP):
\begin{equation}
	\label{eqn_mdp}
	\left(\states, \actions, \transit, \robj \right),
\end{equation}
where:
\begin{enumerate}
\item $\states$ is the \textit{state space}, assumed as a normed vector space of all states of the given environment;
\item $\actions$ is the \textit{action space}, that is a set of all actions available to the agent, it may be discrete or continuous, compact or non-compact;
\item $\transit : \states \times \actions \times \states \ \rightarrow \ \R$ is the \textit{transition probability density function} of the environment, that is such a function that $\transit(\bullet \mid \state_{t}, \action_{t})$ is the probability density of the state $s_{t + 1}$ at step $t+1$ conditioned on the current state $\state_{t}$ and current action $\action_{t}$;
\item $\robj : \states \times \actions \rightarrow \mathbb{R}$ is the reward function of the problem, that is a function that takes a state $\state_{t}$ and an action $\action_{t}$ and returns the immediate reward $\robj_{t}$ incurred upon the agent if it were to perform action $\action_{t}$ while in state $\state_{t}$.
\end{enumerate}

Let $(\Omega, \Sigma, \mathbb P)$ be a probability space underlying \eqref{eqn_mdp}, and $\mathbb E$ be the respective expected value operator.
The problem of reinforcement learning is to find a policy $\policy$ from some space of admissible policies $\policies$ that maximizes 
\begin{equation}
	\label{eqn_value}
	\Value^{\policy}(\state) := \E[\Action \sim \policy]{\sum_{t = 0}^{\infty}\gamma^{t}\robj(\State_{t}, \Action_{t}) \mid \State_0=\state}, \state \in \states	
\end{equation}
for some $\gamma \in (0, 1]$ called a discount factor.
The problem may be concerned with a designated initial state $\state$, a distribution thereof, or even the whole state space.
A policy may be taken as a probability density function or as an ordinary function (cf. Markov policy).
The policy $\policy^*$ that solves the stated problem is commonly referred to as the optimal policy.
An agent will be referred to as a finite routine that generates actions from the observed states.

In some problems, the reward function may have the property that the environment reach the maximal reward being in a certain state or a set thereof \eg the optimal robot routing where the maximal reward is reached at the target state.
For instance, one may assume the reward to be zero at the origin, say, $\state=0$ or some set $\G \subset \states$ and zero action, and strictly negative outside.
When $\G$ is reached by the agent, the environment may be considered \eg solved.
Actually, even if the maximal reward is not reached exactly, a sufficiently large value thereof may be considered acceptable by the user.
So if \eg the target is $\state=0$ and $\robj(0, 0) = 0$, $\robj<0$ otherwise, one may wish to consider environment solved when \eg $\State \in \G, \G \subset \states, 0 \in \G$ almost surely (a.~s.), or in mean etc.
It should be remarked that the user needs not to actually specify $\G$, just the reward function is sufficient to state the problem, whence a set $\G$ occurs naturally.
In general, one may drop some state components from the reward thus restricting goal reaching to a subset of state variables. 
We do not focus on these details here and assume, and, for simplicity, $\G$ to be a compact neighborhood of the origin of the subspace spanned by the state variables of interest.
Notice though that the environment may not necessarily be solved optimally, while respecting the problem of maximizing the value $\Value$.
For instance, a robot may reach the target pose by some agent that produces suboptimal route and possibly unnecessary action effort.
Thus, the problem \eqref{eqn_mdp} may be considered as the problem of reaching (and not leaving) $\G$ optimally in the described context.
Just reaching $\G$ may be done by various classical techniques such as proportional-derivative-integral regulator \cite{Johnson2005PIDcontrol,Wang2020PIDcontrolsys}, sliding-mode regulator \cite{Perruquetti2002SlidingModeCo,vaidyanathan2017applications}, flatness-based regulators \cite{Zhu2006Flatnessbased}, energy-based regulators \cite{Spong1996Energybasedco}, funnel regulators \cite{Berger2021Funnelcontrol}, gain schedulers \cite{Rotondo2017Advancesgains} etc., but doing so optimally is a non-trivial task for which reinforcement learning is currently the most promising approach.
Now, let the goal $\G$ be a compact neighborhood of the origin and the distance to it be denoted $\goaldist(\state) := \inf\limits_{\state' \in \G} \nrm{\state - \state'}$.
Let $\policies_0 \subset \policies$ denote the set of policies which satisfy the following goal reaching property:
\begin{equation}
	\label{eqn_introstab}
	\policy_0 \in \policies_0 \implies \begin{cases}
		\lim\limits_{t \ra \infty}\E[\policy_0]{\goaldist(\State_t)} = 0, \\
		\forall \eps>0 \spc \exists \delta \ge 0 \spc \E{\goaldist(\State_0)} \le \delta \implies \forall t \ge 0 \spc \E[\policy_0]{\goaldist(\State_t)} \le \eps.
	\end{cases}
\end{equation}
That is, $\policies_0$ reaches the goal in mean with a locally bounded overshoot.
In \eqref{eqn_introstab}, it is natural to assert that $\delta$ is unbounded as a function of $\eps$ for otherwise it would not provide a meaningful overshoot bound. 
%Statistical confidence bounds by \eg Hoeffding’s Inequality in terms of the environment episode number \cite{Hertneck2018Learningapprox} can be used to verify a condition of the kind \eqref{eqn_introstab}.
Different probabilistic conditions can also be considered (see \Cref{crl_calfstabevent}, \Cref{lem_calfstabtract}).
%\begin{equation}
%	\label{eqn_introstabalt}
%	\policy_0 \in \policies_0 \implies \PP{\lim\limits_{t \ra \infty}\inf\limits_{\state \in \G} \nrm{\State_t - \state} = 0 \mid \Action_t \sim \policy_0(\bullet \mid \state_t)} \ge 1-\eps, \eps>0.
%\end{equation}
%The results derived in this work hold independent of whether $\policy_0$ satisfies or \eqref{eqn_introstab} or \eqref{eqn_introstabalt}, or any similar goal reaching condition.
Notice $\policies_0$ is problem-specific.
Furthermore, under the properties of the reward function stated above \ie being zero on $\G$ under zero action and strictly negative otherwise, and if $\gamma=1$, the optimal policy $\policy^*$ is in $\policies_0$.
Hence, a generic $\policy_0 \in \policies_0$ is suboptimal by default and a reinforcement learning agent, once reached the performance of such a $\policy_0$ in terms of the value $\Value^{\policy_0}$, will actually seek to improve over it.
Our quest here is to find a way to boost the learning of the said agent while preserving the goal reaching property of $\policy_0$.

==> input/conclusion.tex <==
This work presented an approach to improve agent learning via ensuring a goal reaching property for the stated return maximization problem.
While simply reaching a designated goal (or a goal that arises naturally from the stated reward rate) is not difficult and can be done via numerous techniques, including  proportional-derivative-integral regulator, sliding-mode regulator, flatness-based regulators, energy-based regulators, funnel regulators, gain schedulers etc., doing so optimally is the main challenge addressed by reinforcement learning.
The purpose of this work was to study how goal reaching guarantee could help the agent learning.
A fairly flexible algorithm for this sake was presented and benchmarked on six problems providing an empirical evidence for better learning under the said guarantee.
The algorithm should not necessarily be seen as a direct alternative to, say, proximal policy optimization, and can be built on top of a nominal agent.
Formal analysis of the algorithm was provided.

==> input/contribution.tex <==
This work presents a method of reinforcement learning, which once achieved a goal-reaching property or, alternatively, provided with a policy $\policy_0 \in \policies_0$, preserves the said property in all learning episodes thus serving few-episode learning capabilities and sample efficiency due to avoidance of trials which fail probabilistic goal reaching condition and hence fail to improve the value.
A rigorous mathematical analysis of the said property preservation is provided.
Although not necessarily seen as a direct alternative to such popular baselines as deterministic deep policy gradient (DDPG) and proximal policy optimization (PPO), the demonstration of superiority in learning dynamics is given compared to the said agents, and also to REINFORCE, vanilla policy gradient (VPG) on six environments: cartpole, inverted pendulum, two-tank system, non-holonomic robot, omnidirectional robot (omnibot) and lunar lander.
The statement of not being a direct alternative should emphasize the fact the herein presented approach could also be seen as complementary to \eg PPO \ie it may be integrated into PPO.
The details follow in the main text.
The code for this work is available at \url{https://github.com/osinenkop/regelum-calf}.

==> input/limitations.tex <==
The reference to a policy $\policy_0$ is, strictly speaking, a limitation of \Cref{alg_calfstate}.
However, there are reasons to recommend \Cref{alg_calfstate}.
First, finding $\policy_0$ is commonly not difficult and can be done in a systemic way following one of the established techniques of \eg proportional-derivative-integral regulation, sliding-mode regulation, flatness-based regulation, energy-based regulation, funnel regulation, gain scheduling etc.
The biggest challenge is to optimally solve the environment, which is the target problem of reinforcement learning.
Second, it is generally not possible to guarantee goal reaching by an arbitrary agent in all learning episodes.
It is asserted here that some insight is needed within the agent and a minimalistic one is the reference to $\policy_0$.
Notice that even just a combination of two goal reaching policies, say, $\policy_0, \policy'_0$, is not in general goal reaching as well.
\Cref{alg_calfstate} comprises of a non-trivial integration of $\policy_0$ into the agent by carefully saving the last successful critic update.
Third, our experiments on six problems showed that even pre-trained agents, which achieved the value of the respective $\policy_0$, were mostly beaten by \Cref{alg_calfstate}.
It is thus claimed that at least for the problems, where a policy $\policy_0$ is accessible, agent design as per \Cref{alg_calfstate} may be seen beneficial.

==> input/reproducibility_checklist.tex <==
This paper:

\begin{itemize}
	\item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textbf{yes} \\
	\textit{We give algorithm listings with full details in the main text.}
	\item Clearly delineates statements that are opinions, hypotheses, and speculation from objective facts and results: \textbf{yes} \\ 
	\textit{We formulated main formal claims in theorems with clearly stated hypotheses, kindly refer to the main text.
	Miscellaneous formal results are found in the technical appendix.}
	\item Provides well-marked pedagogical references for less-familiar readers to gain the background necessary to replicate the paper: \textbf{yes} \\
	\textit{We give an overview of the recent state of the art in reinforcement learning in the main body.}
	\item Does this paper make theoretical contributions? \textbf{yes} \\
	\textit{We state them in the main theorem.
	Further results are provided in the technical appendix.}
	\item All assumptions and restrictions are stated clearly and formally:  \textbf{yes} \\
	\textit{They are provided in the statement of the main theorem as technical theorems in the appendix.}
	\item All novel claims are stated formally (e.g., in theorem statements): \textbf{yes} \\
	\textit{Yes, we give the claims in theorems.}
	\item Proofs of all novel claims are included: \textbf{yes}
	\item Proof sketches or intuitions are given for complex and/or novel results: \textbf{yes} \\
	\textit{We intuition in the suggested approach section and in remarks, particularly after the main theorem. We also provide extensive motivation for the new algorithm.}
	\item Appropriate citations to theoretical tools used are given: \textbf{yes} \\ 
	\textit{We provide an overview of popular RL methods, including SAC, PPO, TD3, etc., all of which we studied in our experiments.}
	\item All theoretical claims are demonstrated empirically to hold: \textbf{yes} \\
	\textit{Kindly see our experiments.}
	\item All experimental code used to eliminate or disprove claims is included: \textbf{yes} \\
	\textit{The code is provided with clear instructions on how to use it.}
	\item Does this paper rely on one or more datasets? \textbf{no} \\
	\textit{All the data are generated standalone using the code we provide.}
	\item Does this paper include computational experiments? \textbf{yes} \\ 
	\textit{Kindly refer to the code appendix.}
	\item Any code required for pre-processing data is included in the appendix: \textbf{no} \\
	\textit{Data pre-processing was not relevant to the current study.}
	\item All source code required for conducting and analyzing the experiments is included in a code appendix: \textbf{yes} \\
	\textit{Evaluation results are output upon executing the code.}
	\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes: \textbf{yes} \\
	\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from: \textbf{yes} \\
	\textit{The code is appropriately commented.}
	\item If an algorithm depends on randomness, the method used for setting seeds is described in a way sufficient to allow replication of results: \textbf{yes} \\
	\textit{We describe how we set the seeds.}
	\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks: \textbf{yes} \\
	\textit{The infrastructure details are provided in the code appendix.}
	\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics: \textbf{yes} \\
	\textit{Kindly see the experiment details in the technical appendix.}
	\item This paper states the number of algorithm runs used to compute each reported result: \textbf{yes} \\
	\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank): \textbf{no} \\	
	\textit{The performance improvement is judged by the median learning curves and respective confidence intervals, in particular, final converged values of each agent and learning dynamics}
	\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments: \textbf{yes} \\
	See the experiment details section of the technical appendix.
	\item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting: \textbf{yes.} \\
	\textit{We used default hyperparameters of CleanRL for SAC and TD3, which were considered well-tuned. Otherwise, we used greedy search.}
\end{itemize}

==> input/results.tex <==
Experiments were conducted on six problems with six environments -- cartpole, inverted pendulum, two-tank system, non-holonomic robot, omnidirectional robot (omnibot) and lunar lander -- under five agents: REINFORCE, VPG, DDPG, PPO, and a benchmarked agent following \Cref{alg_calfstate}.
%We used dense quadratic rewards for each problem.
The details of each problem can be found in \Cref{sec_systems}.
%The experiments collectively required approximately 1500 hours of CPU time (on a 3.1 GHz machine) and utilized no more than 1 GB of RAM per thread.
The technical details of the agents may be found in \autoref{sec_experimdetails}.
A policy $\policy_0$ for each environment was designed by energy-based and proportional-derivative-integral regulators.
We aimed to pretrain every benchmarking agent (REINFORCE, VPG, DDPG, PPO) to achieve at least the value of $\policy_0$ in each experiment.
The learning curves of the agents, which succeeded in this task, are shown in \Cref{fig_learncurves}.
The accumulated rewards are shown relative to the one achieved by using $\policy_0$.
Hence, the plots essentially show how much better than $\policy_0$ the agents performed.
The respective numerical values are given in \Cref{tab_accummedians}.
More detailed evaluation data are provided in \autoref{sec_rawresults}.
We observed learning convergence for lunar lander by PPO and VPG in about 500k agent-environment interaction steps -- similar results were reported \eg in \cite{Huang2024PPOClipAttain,Park2024UnveilingSigni}. 
%These results are in sync with findings from other studies \cite{Park2024UnveilingSigni}. 
%We also observed that PPO on the Lunar Lander environment converged in about 500k timesteps, aligning well with previous work. 
For the inverted pendulum environment, it was reported that PPO required approximately 85k timesteps to achieve convergence \cite{Yang2022Policyoptimiza}. 
Our results showed that PPO converged in about 90--100k steps, which is consistent with the said existing benchmark.
For the cartpole, around 80--100k steps total was needed for PPO to converge as reported in \cite{He2022Representation,IshidaLangPropcodeo}.
In our studies, such performance was achieved on separate runs, but about 300--400k was required in median.
Nevertheless, the agent by \Cref{alg_calfstate} required not more than 10k steps in median which is superior anyway, justifying the claim of the work.
Overall, we observed superior performance of the agent by \Cref{alg_calfstate} in all problems, except for the lunar lander.
Nevertheless, in terms of the total learning iterations, the agent by \Cref{alg_calfstate} was still superior as it required no pretraining.
Notice \Cref{fig_learncurves} shows all learning iterations of the agent by \Cref{alg_calfstate}.

%\blue{Lander reported results for PPO on the Lunar Lander environment, showing that about 500-600k timesteps were required for convergence \cite{Huang2024PPOClipAttain}. 
%These results are in sync with findings from other studies \cite{Park2024UnveilingSigni}. 
%In our experiments, we observed that PPO on the Lunar Lander environment converged in about 500k timesteps, aligning well with previous work. 
%For the Inverted Pendulum environment, another work reported that PPO required approximately 85k timesteps to achieve convergence \cite{Yang2022Policyoptimiza}. 
%Our results showed that PPO converged in about 100k timesteps, which is consistent with the existing benchmark.
%}
% \blue{Comparison with other reported results: around 80-100k time steps total was needed for PPO to converge on cartpole \cite{He2022Representation,IshidaLangPropcodeo}.
% Our result is not on par with this.
% Check!
% Lander reported results for PPO: about 500-600k time steps until convergence \cite{Huang2024PPOClipAttain}.
% This in synced with another work: \cite{Park2024UnveilingSigni}.
% Our results for PPO?
% PPO on inv pendulum: about 85k time steps \cite{Yang2022Policyoptimiza}.
% Ours: about 30-50 iters for DDPG, PPO.
% How many time steps?
% }

\begin{table*}[t]
\caption{Medians of accumulated rewards upon convergence for various algorithms relative to the baseline policy $\policy_0$, with $\policy_0$'s performance subtracted from each algorithm's performance.}
\label{tab_accummedians}
\centering
\begin{tabular}{lllllll}
	\toprule
	 & Inverted & 2-tank & 3-wheeled & Cartpole & Lunar & Omnibot \\
	 & pendulum & system & robot &  & lander &  \\
	\midrule
	REINFORCE & 40.3 & 51.0 & 97.4 & -514.8 & -5.6 & 1010.5 \\
	DDPG & 28.8 & 33.5 & -780.3 & -2036.7 & -131.0 & 1239.9 \\
	VPG & -219.1 & 35.9 & 194.2 & -809.9 & \textbf{43.2} & 1213.7 \\
	PPO & 51.2 & -79.6 & -69.7 & 102.9 & 34.8 & 597.7 \\
	Agent by \Cref{alg_calfstate} & \textbf{56.0} & \textbf{55.0} & \textbf{196.2} & \textbf{111.9} & 6.4 & \textbf{1271.1} \\
	% \midrule
	% $\policy_0$ & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
	% \midrule
	% MPC (horizon 3) & -419.7 & 55.1 & 282.0 & 103.4 & 44.1 & 1328.2 \\
	% MPC (horizon 7) & -120.8 & 55.3 & 282.0 & 109.6 & 56.2 & 1328.2 \\
	% MPC (horizon 11) & -30.1 & 55.4 & 282.5 & 110.9 & 47.8 & 1328.2 \\
	\bottomrule
	\end{tabular}
\end{table*}

\begin{figure*}[t]
\centering
\centerline{\includegraphics[width=\textwidth]{gfx/learning_curves.pdf}}
\caption{Smoothed learning curves\ie accumulated reward vs. iterations.
The plots represent median performance relative to the baseline policy $\policy_0$, with the accumulated reward of $\policy_0$ subtracted for clarity. 
The iterations axis is human-normalized (see \Cref{sec_rawresults} for unnormalized plots). 
Plots are truncated starting when policy gradient algorithms (PPO, DDPG, VPG, REINFORCE) reach $\pi_0$ performance, while full learning plots are shown for agent by \Cref{alg_calfstate}.
% Plots are smoothed using \texttt{uniform\_filter1d}, with B\'ezier interpolation applied to CALF.}
}

\label{fig_learncurves}
\end{figure*}
	


==> input/sota.tex <==
Common reinforcement learning approaches to the above stated problem include various tabular dynamic programming, episodic Monte-Carlo and online methods (see \eg \cite{Sutton2018ReinforcementL,Bertsekas2019Reinforcementl,Lewis2013Reinforcementl,Vrabie2012OptimalAdaptiv,Bouzy2006MonteCarloGo,Lazaric2007Reinforcementl,Vodopivec2017montecarlotre} for overviews).
Applications range from robotics \cite{Kumar2016Optimalcontrol,Borno2013TrajectoryOpti,Tassa2012Synthesisstabi,Surmann2020DeepReinforcem,Akkaya2019Solvingrubiks} to games such as Go, chess, shogi (also known as Japanese chess) \cite{Silver2016Masteringgame,Silver2018generalreinfor}, and even complex video games such as StarCraft II \cite{Vinyals2019Grandmasterlev}.

Some simple policy gradients \cite{Baxter2001Infinitehorizo,Sutton1999PolicyGradient,Williams1992Simplestatisti,Kakade2001naturalpolicy,Peters2006Policygradient}, like REINFORCE, are almost direct adaptations of the stochastic approximation theory, whereas advanced methods employ sophisticated step size adjustments, critic learning, batch sampling techniques etc.
The contemporary progress in refinement and improvement of reinforcement learning agents is fairly active.
Among the most profound basis methods of reinforcement learning are deterministic policy gradient (DDPG) \cite{Silver2014DeterministicP} and proximal policy optimization (PPO) \cite{Schulman2017ProximalPolicy}.
In particular, DDPG is suitable for problems with continuous action spaces commonly found in \eg robotics \cite{Lillicrap2016Continuouscont}.
Implementation tweaks, such as value, gradient and reward clipping; reward and layer scaling were studied in trust region policy optimization and PPO \cite{Engstrom2019Implementationa}.

It was shown that without the said tweaks, PPO was similar to trust region policy optimization in performance.
In the experiments of this work, the described tweaks were employed, particularly layer scaling for the actor neural network output.
Furthermore, generalized advantage estimation (GAE) in vanilla policy gradient (VPG) and PPO was employed for tackling the common pitfalls of value loss clipping  \cite{Schulman2018HighDimensiona,Andrychowicz2020Whatmatterspo,Huang2024PPOClipAttain}.
Large batches have consistently been reported to produce better agent neural network convergence up until recently \cite{Nikulin2023QEnsembleOffl,Akimov2023LetOfflineRL,Nikulin2023AntiExploratio,You2020LargeBatchOpt,Ginsburg2018LargeBatchTra}.
In all studied baselines of this work, samples from the replay buffers were taken large (larger than 256), as recommended.
Besides GAE, there are various tuning recommendations which were also employed following \cite{Furuta2021CoAdaptationA,Engstrom2020Implementation,Paine2020Hyperparameter,Yang2020OfflinePolicy,Henderson2019DeepReinforcem}.
Policy iteration format critic learning, inspired by \cite{Song2019Vmpopolicy}, was reported to help stabilize policy gradients without the need for excessive entropy tuning.
This was employed in the studied baselines as well.

Exploration reinforcement learning presents its own challenges, as highlighted by \cite{Wang2020Strivingsimpli}.
They show that squashed actions can lead to poor exploration.
In the current work, this was avoided by using a truncated normal distribution for action selection to ensure more natural exploration behaviors.
This decision is informed by the discussion in \cite{Fujita2018Clippedaction}, which suggested that without such a distribution, one might encounter problematic Q-function estimations.

The significance of $N$-step returns in enhancing learning with large replay buffers should also be noted \cite{Fedus2020Revisitingfund}.
Their research suggested that uncorrected $N$-step returns could be beneficial for replay strategy.

Up-to-date performance on some popular problems relevant to this study should be mentioned.
So \eg PPO required 500k agent-environment interaction steps as reported \eg in \cite{Huang2024PPOClipAttain,Park2024UnveilingSigni}. 
%These results are in sync with findings from other studies \cite{Park2024UnveilingSigni}. 
%We also observed that PPO on the Lunar Lander environment converged in about 500k timesteps, aligning well with previous work. 
For the inverted pendulum environment, this number was reported to be about 80k \cite{Yang2022Policyoptimiza}. 
%Our results showed that PPO converged in about 90--100k steps, which is consistent with the said existing benchmark.
For the cartpole, around 80--100k steps total was needed for PPO to converge as reported in \cite{He2022Representation,IshidaLangPropcodeo}.
The studies in \Cref{sec_results} indicate good alignment with these numbers with the newly suggested agent greatly outperforming the baselines on five out of six problems.
%In our studies, such performance was achieved on separate runs, but about 300--400k was required in median.
%Nevertheless, the agent by \Cref{alg_calfstate} required not more than 10k steps in median which is superior anyway, justifying the claim of the work.

==> input/stabilizers.tex <==
\subsection{The baseline goal-reaching policies $\pi_0$}

\subsubsection{Omnibot (kinematic point)}

\begin{equation}
    a = \begin{pmatrix} 
        -0.5 x \\ -0.5 y
    \end{pmatrix}
\end{equation}

\subsubsection{Pendulum}

\begin{equation}
    a = 
    \begin{cases}
    	0.03\sgn\left(\frac{mgl\omega}{2}  (\cos(\vartheta) - 1) + \frac{m l^ 2\omega^3}{6}\right), \text{ if } \cos\vartheta \leq \cos(\pi / 10) \lor |\omega| > 0.2 \\
    	0.6 \sin(\vartheta) + 0.2 \omega, \text{ otherwise}
    \end{cases}
\end{equation}

\subsubsection{Inverted Pendulum}

\begin{equation}
    a = (1 - \lambda)a_{\text{upswing}} + \lambda a_{\text{upright}}  
\end{equation}
where
\begin{itemize}
    \item $a_{\text{upright}} = 70 \vartheta + 20 \omega$ 
    \item $a_{\text{upswing}} = \begin{cases} 3\sign(\omega), \text{ if } \cos\vartheta < 0 \\ 3\sign(\sin\vartheta), \text{ otherwise } \end{cases}$
    \item $\lambda = \frac{1 - \tanh\left(\frac{\vartheta - 0.35}{10}\right)}{2}$    
\end{itemize}

\subsubsection{Three-wheel robot}

\begin{equation}
    a =
    \begin{cases}
        \begin{pmatrix}
            0 \\ - 3 \sign(\vartheta - \atantwo(y, x)) \sqrt{|\vartheta - \atantwo(y, x)|}
        \end{pmatrix}, \\ \qquad\qquad\qquad\qquad \begin{aligned} & \text{if } (|x| \geq 0.001 \lor |y| \geq 0.001) \land \\ & (|\vartheta - \atantwo(y, x)| \geq 0.001), \end{aligned} \\ 
        \begin{pmatrix}
            - 3 \sqrt[4]{x ^ 2 + y ^ 2} \\ 0
        \end{pmatrix},  \begin{aligned} & \text{ if } (|x| \geq 0.001 \lor |y| \geq 0.001) \land \\ & (|\vartheta - \atantwo(y, x)| < 0.001) \end{aligned} \\
        \begin{pmatrix}
            - 0 \\ - 3 \sign{\vartheta} \sqrt{|\vartheta|}
        \end{pmatrix}, \text{ if } (|x| < 0.001 \lor |y| < 0.001) \land (|\vartheta| >= 0.001) \\
        \begin{pmatrix}
            0 \\ 0
        \end{pmatrix}, \text{ otherwise } 
    \end{cases}
\end{equation}

\subsubsection{Two-tank system}

\begin{equation}
    a = \frac{-6.5 (h_1 - 0.4) + \frac{2h_1}{\tau_1} - 6.5 (h_2 - 0.4) - 2\left( -h_1 + K_2 h_1 + K_3 h_2^2 \right)}{1 + \frac{2K_1}{\tau_1}}
\end{equation}

\subsubsection{Lunar lander}

\begin{equation}
    a = \begin{pmatrix}
        -80 \vartheta - 20 \omega - \cos^2\vartheta (-10 x - 40 v_x )  \\ 0
    \end{pmatrix}
\end{equation}
